NuGrid Stellar Data Set. II. Stellar Yields from H to Bi for Stellar Models with Mzams = 1 to 25Msun and Z = 0.0001 to 0.02

We provide here a significant extension of the NuGrid Set 1 models in mass coverage and toward lower metallicity, adopting the same physics assumptions. The combined data set now includes the initial masses M/Msun = 1, 1.65, 2, 3, 4, 5, 6, 7, 12, 15, 20, 25 for Z = 0.02, 0.01, 0.006, 0.001, 0.0001 with alpha-enhanced composition for the lowest three metallicities. These models are computed with the MESA stellar evolution code and are evolved up to the AGB, the white dwarf stage, or until core collapse. The nucleosynthesis was calculated for all isotopes in post-processing with the NuGrid mppnp code. Explosive nucleosynthesis is based on semi-analytic 1D shock models. Metallicity-dependent mass loss, convective boundary mixing in low- and intermediate mass models and H and He core burning massive star models is included. Convective O-C shell mergers in some stellar models lead to the strong production of odd-Z elements P, Cl, K and Sc. In AGB models with hot dredge-up the convective boundary mixing efficiency is reduced to accommodate for its energetic feedback. In both low-mass and massive star models at the lowest metallicity H-ingestion events are observed and lead to i-process nucleosynthesis and substantial N-15 production. Complete yield data tables, derived data products and online analytic data access are provided.

==> tables/compareOtherWork_M15_set1_5a.tex <==
\begin{table}
\begin{center}
\caption{Comparison of the total ejecta of $\mzams=15\msun$, $Z=0.0001$ models from this work (delay),
CL04 and K06.}
\begin{tabular}{ccccc}
\hline
\hline
specie & delay & CL04      & K06        \\ 
\hline
 C-12   & 1.646E-01           & 1.635E-01           & 2.000E-01  \\ 
 C-13   & 3.145E-06           & 1.473E-05           & 4.980E-06  \\ 
 N-14   & 3.048E-04           & 3.156E-04           & 3.370E-04  \\ 
 N-15   & 1.994E-07           & 2.322E-05           & 6.760E-08  \\ 
 O-16   & 1.176E+00           & 8.888E-01           & 4.590E-01  \\ 
 O-17   & 3.761E-06           & 3.572E-06           & 3.980E-06  \\ 
 O-18   & 3.643E-06           & 5.752E-06           & 7.130E-06  \\ 
 F-19   & 4.664E-08           & 7.342E-06           & 1.870E-08  \\ 
 Ne-20  & 1.468E-01           & 6.007E-02           & 4.240E-02  \\ 
 Na-23  & 5.355E-04           & 1.002E-04           & 1.840E-04  \\ 
 Mg-24  & 7.140E-02           & 5.186E-02           & 5.410E-02  \\ 
 Al-27  & 1.159E-03           & 6.400E-04           & 5.500E-04  \\ 
 Si-28  & 1.038E-01           & 1.273E-01           & 1.140E-01  \\ 
 S-32   & 4.318E-02           & 6.790E-02           & 4.900E-02  \\ 
 Ar-36  & 7.312E-03           & 1.377E-02           & 8.940E-03  \\ 
 Ca-40  & 5.110E-03           & 1.093E-02           & 7.710E-03  \\ 
 Ti-48  & 2.847E-04           & 2.883E-04           & 1.830E-04  \\ 
 V-51   & 1.479E-04           & 3.215E-05           & 8.020E-06  \\ 
 Cr-52  & 3.226E-03           & 3.171E-03           & 1.790E-03  \\ 
 Mn-55  & 3.858E-04           & 7.202E-04           & 3.990E-04  \\ 
 Fe-56  & 6.649E-02           & 1.422E-01           & 1.000E-01  \\ 
 Co-59  & 5.606E-04           & 1.610E-03           & 3.500E-05  \\ 
 Ni-58  & 6.217E-02           & 2.157E-03           & 3.110E-04  \\ 
 Zn-70  & 1.691E-06           & 5.168E-05           & 9.570E-10  \\ 
 Ge-70  & 5.790E-06           & 1.207E-04           & 3.360E-09  \\ 
 Se-76  & 2.245E-06           & 3.338E-05           & 8.930E-10  \\ 
 Kr-80  & 1.857E-08           & 3.285E-06           & 2.500E-10  \\ 
 Kr-82  & 1.473E-07           & 3.346E-06           & 9.080E-10  \\ 
 Sr-86  & 1.336E-07           & 3.228E-06           & 4.670E-10  \\ 
 Sr-87  & 1.005E-07           & 2.295E-06           & 2.540E-10  \\ 
 Sr-88  & 5.325E-05           & 1.832E-03           & 2.970E-09  \\ 
\hline
\noalign{\smallskip}
\hline
\end{tabular}
\label{compareOtherWork_M15_set1_5a}
\end{center}
\end{table}


==> tables/massive_star_properties_table.tex <==
%Complete tables for online version

%Table 8 in paper
\begin{table}
\caption{Final core masses $M_{\mathrm{final}}$ and total lifetime 
$\tau_{\mathrm{total}}$ for $Z=0.0001$.}
\center
\begin{tabular}{lrr}
initial mass & $M_{\mathrm{Final}}$ & $\tau_{\mathrm{total}}$ \\
\hline
 [$\msun$]           & [$\msun$] & [$yr$] \\
\hline
\multicolumn{3}{c}{Z=0.0001} \\
\hline
1.0 & 0.592 & 5.670E+09 \\
1.65& 0.637 & 1.211E+09 \\
2.0 & 0.665 & 6.972E+08 \\
3.0 & 0.852 & 2.471E+08 \\
4.0 & 0.905 & 1.347E+08 \\
5.0 & 0.992 & 8.123E+07 \\
6.0 & 1.125 & 5.642E+07 \\
7.0 & 1.272 & 4.217E+07 \\
\hline
\multicolumn{3}{c}{Z=0.001} \\
\hline
1.0 | 5.845E-01 | 6.171E+09 \\
1.65 | 6.169E-01 | 1.069E+10 \\
2.0 | 6.352E-01 | 8.592E+08 \\
3.0 | 8.242E-01 | 2.987E+08 \\
4.0 | 8.936E-01 | 1.518E+08 \\
5.0 | 9.855E-01 | 9.316E+07 \\
6.0 | 1.122E+00 | 6.388E+07 \\
7.0 | 1.259E+00 | 4.710E+07 \\
\hline
\multicolumn{3}{c}{Z=0.006} \\
\hline
1.0 | 5.678E-01 | 8.248E+09 \\
1.65 | 6.140E-01 | 1.644E+09 \\
2.0 | 6.176E-01 | 1.129E+09 \\
3.0 | 7.097E-01 | 3.639E+08 \\
4.0 | 8.611E-01 | 1.727E+08 \\
5.0 | 9.533E-01 | 1.026E+08 \\
6.0 | 1.053E+00 | 6.880E+07 \\
7.0 | 1.164E+00 | 4.971E+07 \\
\end{tabular}\label{tab:cores_agb}
\end{table}

% TAble 10 in paper
\begin{table}
\caption{Lifetimes of major central burning stages of massive star models.
Shown are lifetimes for H burning, $\tau_{\mathrm{H}}$, He burning, $\tau_{\mathrm{He}}$, C burning, $\tau_{\mathrm{C}}$,
Ne burning $\tau_{\mathrm{Ne}}$, O burning, $\tau_{\mathrm{O}}$, Si burning, $\tau_{\mathrm{Si}}$, and the total lifetime
of the stellar models, $\tau_{\mathrm{total}}$. Times in yr.}
\center
\begin{tabular}{lrrrrrrr}
\hline
Model & $\tau_{\mathrm{H}}$ & $\tau_{\mathrm{He}}$ & $\tau_{\mathrm{C}}$ & $\tau_{\mathrm{Ne}}$ & $\tau_{\mathrm{O}}$ & $\tau_{\mathrm{Si}}$ & $\tau_{\mathrm{total}}$\\
\hline
\multicolumn{8}{c}{Z = 0.02} \\
\hline
12  & 1.742E+07 & 1.669E+06 & 1.046E+04 & 1.046E+01 & 2.973E+00 & 1.895E-01 & 1.935E+07\\
15  & 1.243E+07 & 1.250E+06 & 1.835E+03 & 2.829E+00 & 1.361E+00 & 8.840E-02 & 1.386E+07\\
20  & 8.687E+06 & 8.209E+05 & 1.270E+02 & 1.811E+00 & 7.086E-01 & 5.071E-02 & 9.596E+06\\
25  & 6.873E+06 & 6.426E+05 & 2.525E+02 & 5.303E-01 & 1.390E-01 & 1.385E-02 & 7.585E+06\\
\hline
\multicolumn{8}{c}{Z = 0.01} \\
\hline
12  & 1.787E+07 & 1.665E+06 & 1.783E+03 & 6.104E+00 & 3.196E+00 & 1.401E-01 & 1.971E+07\\
15  & 1.290E+07 & 1.223E+06 & 2.881E+03 & 1.446E+00 & 1.735E+00 & 9.452E-02 & 1.423E+07\\
20  & 8.979E+06 & 8.156E+05 & 1.788E+03 & 3.680E-01 & 2.249E-01 & 2.540E-02 & 9.922E+06\\
25  & 7.140E+06 & 6.457E+05 & 3.905E+02 & 6.256E-01 & 6.091E-01 & 4.463E-02 & 7.859E+06\\
\hline
\multicolumn{8}{c}{Z = 0.006} \\
\hline
12  & 1.795E+07 & 1.670E+06 & 4.345E+03 & 1.219E+01 & 3.376E+00 & 2.414E-01 & 1.981E+07\\
15  & 1.296E+07 & 1.218E+06 & 3.751E+02 & 9.122E-01 & 8.084E-01 & 5.914E-02 & 1.436E+07\\
20  & 9.141E+06 & 8.262E+05 & 8.429E+02 & 4.553E-01 & 2.433E-01 & 2.638E-02 & 1.005E+07\\
25  & 7.250E+06 & 6.405E+05 & 1.567E+02 & 6.077E-01 & 1.114E+00 & 8.914E-02 & 7.949E+06\\
\hline
\multicolumn{8}{c}{Z = 0.001} \\
\hline
12  & 1.782E+07 & 1.678E+06 & 1.114E+03 & 2.351E+00 & 2.145E+00 & 1.010E-01 & 1.966E+07\\
15  & 1.305E+07 & 1.178E+06 & 2.999E+02 & 9.481E-01 & 6.948E-01 & 4.270E-02 & 1.433E+07\\
20  & 9.183E+06 & 7.925E+05 & 6.678E+02 & 1.268E+00 & 1.433E-01 & 2.576E-02 & 1.008E+07\\
25  & 7.295E+06 & 6.184E+05 & 1.265E+02 & 4.622E-01 & 6.535E-01 & 8.337E-02 & 7.994E+06\\
\hline
\multicolumn{8}{c}{Z = 0.0001} \\
\hline
12  & 1.750E+07 & 1.550E+06 & 9.097E+02 & 1.294E+00 & 1.922E+00 & 7.426E-02 & 1.925E+07\\
15  & 1.288E+07 & 1.122E+06 & 3.196E+02 & 1.167E+00 & 7.034E-01 & 4.253E-02 & 1.413E+07\\
20  & 9.151E+06 & 7.558E+05 & 3.567E+02 & 1.068E+00 & 1.711E-01 & 2.190E-02 & 9.982E+06\\
25  & 7.284E+06 & 5.952E+05 & 4.199E+02 & 4.468E-01 & 6.640E-01 & 8.287E-02 & 7.927E+06\\
\hline
\end{tabular}\label{tab:lifetimesmassive}
\end{table}






